UNIC: Universal Classification Models via Multi-teacher Distillation

Pretrained models have become a commodity and offer strong results on a broad range of tasks. In this work, we focus on classification and seek to learn a unique encoder able to take from several complementary pretrained models. We aim at even stronger generalization across a variety of classification tasks. We propose to learn such an encoder via multi-teacher distillation. We first thoroughly analyse standard distillation when driven by multiple strong teachers with complementary strengths. Guided by this analysis, we gradually propose improvements to the basic distillation setup. Among those, we enrich the architecture of the encoder with a ladder of expendable projectors, which increases the impact of intermediate features during distillation, and we introduce teacher dropping, a regularization mechanism that better balances the teachers' influence. Our final distillation strategy leads to student models of the same capacity as any of the teachers, while retaining or improving upon the performance of the best teacher for each task. Project page and code: https://europe.naverlabs.com/unic

==> Makefile <==
# where the paper will be compiled
OUTPUT_DIR=/tmp/unic
MAIN_PDF_NAME=unic_eccv2024.pdf

OS_NAME := $(shell uname -s | tr A-Z a-z)
ifeq ($(OS_NAME), linux)
	VIEWER := okular
else
	VIEWER := open -a Skim.app
endif


LATEXMK_VERSION := $(shell latexmk --version 2>/dev/null)


define compile_latexmk
	# argument - 1: filename
	mkdir -p ${OUTPUT_DIR}
	latexmk -pdf -pdflatex="pdflatex --shell-escape" -bibfudge -output-directory=${OUTPUT_DIR} $(1)
endef


define compile_pdflatex
	# argument - 1: filename
	mkdir -p ${OUTPUT_DIR}
	pdflatex -output-directory=${OUTPUT_DIR} -jobname=$(1) $(1)
	openout_any=a bibtex ${OUTPUT_DIR}/$(1)
	pdflatex -output-directory=${OUTPUT_DIR} -jobname=$(1) $(1)
	pdflatex -output-directory=${OUTPUT_DIR} -jobname=$(1) $(1)
endef


.PHONY: main sup view clean os


# target to compile only the main paper
main:
	@echo $@
	@echo "latexmk version: $(LATEXMK_VERSION)"

	# if latexmk is installed, use that
ifdef LATEXMK_VERSION
	$(call compile_latexmk,main)
else
	# otherwise, call pdflatex 3 times
	$(call compile_pdflatex,main)
endif

	# make a copy of the paper with the target file name
	cp ${OUTPUT_DIR}/main.pdf ${MAIN_PDF_NAME}


# target to copy the pdf to Bulent's i-cloud
ic:
	@echo $@

	for fname in "${MAIN_PDF_NAME}" ; do \
		if [ -f $${fname} ]; then \
			cp $${fname} "$${MY_ICLOUD}/"; \
		fi \
	done

# target to visualize the compiled pdf
view:
	@echo "Viewer: $(VIEWER)"
	# $(VIEWER) ${MAIN_PDF_NAME} &
	$(VIEWER) ${OUTPUT_DIR}/main.pdf &


# target to clean up the build directory
clean:
	rm -rf ${OUTPUT_DIR}
	rm paper-figure*


sync:
	git pull --ff
	git push

# target to convert SVG's into PDFs
svg:
	@echo "Converting SVGs into PDFs"

	for sf in "teaser" "clf-standard" "clf-oca" "clf-ocm" "clf-ogc" "augmentations" "projectors" ; do \
		echo "Converting $${sf}" ; \
		inkscape --export-dpi=5000 --export-filename=res/$${sf}.pdf res/$${sf}.svg ; \
	done


# target to print the OS name
os:
	@echo $(OS_NAME)


==> tex/88_protocol.tex <==
\section{Distillation and evaluation protocol}

\subsection{Distillation protocol}
\label{sec:distil_protocol}

\paragraph{Details on the basic setup.} We set projector heads to be Multi-Layer Perceptrons (MLPs) with two hidden layers, GeLU non-linearity and hidden dimension of $d_h$. The default value for $d_h$ is set to $4\times$ the input dimension.



\paragraph{Teachers.}
We use the following model groups as teachers:
\begin{itemize}
    \item \textbf{Self-supervised models}: We use DINO~\cite{caron2021emerging} and iBOT~\cite{zhou2021ibot}, two popular models that have proven extremely effective for generalization.
    DINO is based on contrastive learning, while iBOT uses masked modeling.
    These two learning paradigms have been shown to yield complementary characteristics~\cite{wei2022contrastive,shi2023hybrid}, \ie iBOT has stronger patch token features than DINO, and shows improved performance on dense prediction.
    \item Highly optimized \textbf{supervised models}: We use DeiT-III~\cite{touvron2022deitiii} and a fine-tuned dBOT~\cite{liu2024dbot} that achieve  state of the art top-1 accuracy for ImageNet-1K with a ViT-B architecture, \ie they report 83.8 and 84.5\% top-1 accuracy, respectively.
\end{itemize}


\paragraph{Tasks}
We evaluate our visual encodes in a suite of tasks, that span five axes:
\begin{itemize}
    \setlength\itemsep{0pt}
    \item Image classification on ImageNet-1K~\cite{dosovitskiy2021an} (1000 classes).
    \item Transfer learning on 15 different image classification datasets, that consider diverse sets of concepts. These include the 5 ImageNet-CoG datasets~\cite{sariyildiz2021concept} that are tailored for concept generalization, 8 common small-scale fine-grained datasets (Aircraft, Cars196, DTD, EuroSAT, Flowers, Pets, Food101, SUN397) and two long-tail recognition datasets (iNaturalist-2018 and 2019). We group all such datasets into a set for reporting results, \ie we average performance over all datasets.
    \item Semantic segmentation on the ADE-20k dataset~\cite{zhou2019semantic}.
    \item Depth estimation on the NYUD dataset~\cite{silberman2012indoor}.
\end{itemize}


\subsection{Evaluation protocol}
\label{sec:eval_protocol}

We measure top-1 accuracy for classification tasks, mIoU for semantic segmentation and RMSE for depth.
We measure performance on all tasks after\textit{linear probing}, \ie we learn classifiers for each dataset over the outputs of the student encoder $s$. Note that in this case no teacher specific parameters are used, \ie the representation is fully shared across all tasks. We report results for each of the four tasks described above. For the image classification scenarios we always first extract features and the learn logistic regression classifiers per dataset. For the transfer learning task, we average Top-1 Accuracy over all 15 datasets and report a single metric for mean accuracy. For the dense prediction tasks, we follow the protocol described in the DINOv2 paper~\cite{oquab2023dinov2} and learn per token classifiers for semantic segmentation and depth estimation.

\textit{Plug-and-play} is a scenario where we pair the student output with the pre-existing classifiers that come with the DeiT-III model/teacher. In this case, we append the DeiT-specific projectors over the student encoder for \divine models. \alert{we also report results with similar classifiers for dense prediction that are learned on top of the teacher model.}



==> tex/float/fig_dinodbot_2d_plots.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{.48\textwidth}
        \centering
        \input{tex/float/fig_dinodbot_2d_gen_im1k_plot.tex}
        \caption{Generalization ($\uparrow$) vs. ImageNet ($\uparrow$)}
        \label{fig:dinodbot_2d_gen_im1k}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.48\textwidth}
        \centering
        \input{tex/float/fig_dinodbot_2d_seg_depth_plot.tex}
        \caption{Segmentation ($\uparrow$) vs. depth ($\downarrow$)}
        \label{fig:dinodbot_2d_seg_depth}
    \end{subfigure}
    \caption{
        \textbf{Performance on classification and dense prediction tasks}.
        Note that depth is measured by RMSE where a lower value is better.
        Markers with a triangle denote models distilled from the respective teachers (DINO, dBOT-ft) in a basic way, \ie from a single teacher.
    }
    \label{fig:dinodbot_2d_plots}
\end{figure}


==> tex/float/fig_dinodeit_2d_plots.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{.48\textwidth}
        \centering
        \input{tex/float/fig_dinodeit_2d_gen_im1k_plot.tex}
        \caption{Generalization ($\uparrow$) vs. ImageNet ($\uparrow$)}
        \label{fig:dinodeit_2d_gen_im1k}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{.48\textwidth}
        \centering
        \input{tex/float/fig_dinodeit_2d_seg_depth_plot.tex}
        \caption{Segmentation ($\uparrow$) vs. depth ($\downarrow$)}
        \label{fig:dinodeit_2d_seg_depth}
    \end{subfigure}
    \caption{
        \textbf{Performance on classification and dense prediction tasks}.
        Note that depth is measured by RMSE where a lower value is better.
        Markers with a triangle denote models distilled from the respective teachers (DINO, DeiT-III) in a basic way, \ie from a single teacher.
    }
    \label{fig:dinodeit_2d_plots}
\end{figure}


==> tex/float/fig_dp_linprob.tex <==

\begin{tikzpicture}[trim axis right,trim axis left]
\begin{axis}[
    xlabel={Epoch},
    ylabel={Loss},
    ymin=0.1, ymax=0.4,
    width=1.1\linewidth,
    height=4cm,
    grid=major,
    label style={font=\scriptsize},
    tick label style={font=\scriptsize},
    legend style={at={(0.05, 0.05)}, anchor=south west, legend columns=1, font=\tiny},
]






\end{axis}
\end{tikzpicture}



